GSP - The Cinderella of Mechanism Design

Nearly fifteen years ago, Google unveiled the generalized second price (GSP) auction. By all theoretical accounts including their own [Varian 14], this was the wrong auction --- the Vickrey-Clarke-Groves (VCG) auction would have been the proper choice --- yet GSP has succeeded spectacularly. We give a deep justification for GSP's success: advertisers' preferences map to a model we call value maximization, they do not maximize profit as the standard theory would believe. For value maximizers, GSP is the truthful auction [Aggarwal 09]. Moreover, this implies an axiomatization of GSP --- it is an auction whose prices are truthful for value maximizers --- that can be applied much more broadly than the simple model for which GSP was originally designed. In particular, applying it to arbitrary single-parameter domains recovers the folklore definition of GSP. Through the lens of value maximization, GSP metamorphosizes into a powerful auction, sound in its principles and elegant in its simplicity.

==> objectives.tex <==


\section{Advertisers and their Objectives}  \label{sec:obj}

We briefly introduced a handful of reasons that revenue maximization is a better model of an advertiser's preferences. We discuss those in detail here.

\subsection{Return on Investment (ROI) Constraints}

In marketing, the cost-benefit trade-off is generally measured by an advertiser's return on investment (ROI). Whereas profit measures the difference between value and cost, the ROI depends on the ratio. This somewhat small change results in manifestly different applications; ROI becomes a constraint instead of an objective, naturally leading advertisers to maximize revenue.

Profit is a standard objective in theory. For an agent with value $v$ who pays cost $p$, the profit is simply
\[Profit=v-p\enspace.\]
Profit maximization is consistent with standard quasi-linear utility functions ($u=v-p$) and is well-studied.

In contrast, advertisers usually measure ROI. Again considering an agent who gets value $v$ and pays price $p$, the ROI is given by
\[ROI=\frac{v-p}{p}=\frac{v}{p}-1\enspace.\]
Because ROI is a density measure (value per unit spend), it does not make sense to optimize for it directly; rather, ROI is manifested as a constraint.

Sponsored search illustrates the senslessness of optimizing for ROI. Note that an advertiser in sponsored search can get clicks at a very low price per click simply by being the lowest ad on the page; however, while this will maximize ROI, the advertiser will get very few clicks this way. This is not what advertisers want.


It remains to build preferences with ROI constraints. Since costs are already included through the ROI constraint, the most basic model says that an advertiser's objective should not depend on costs, i.e. the advertiser should maximize revenue. Thus, we argue that {\em value maximization with a ROI constraint} is the natural fundamental model for an anyone whose costs are primarily accounted for in ROI metrics.

That said, ROI constraints can be added to any model of preferences. As we will see later, these have 



\subsection{Budgets and Fiat Money}

Value maximization is a natural model when agents have no value for money, which is commonly true of marketers.

The standard model of quasi-linear preferences supposes that an agent gets utility from having unspent budget. This captures the idea that the bidder has outside options on which that money can be spent. (In our world with fiat money, money technically has no value beyond the fact that it can be spent on things.)

In contrast, an agent who prefers revenue does not care about how much money is left over insofar as constraints are not violated. Those constraints (ROI and budget) serve to make sure that the final outcome is acceptable to the advertiser.

In marketing, 



\subsection{Average-Centric Targets}

The metrics and tools used by advertisers correspond to revenue maximization, not profit maximization. A quick survey 

\begin{itemize}
\item Advertiser analysis tools universally report average costs
\item Yahoo
\item Google
\item ???
\end{itemize}


\subsection{Value Uncertainty}

The standard theory assumes 


